TS-UCB: Improving on Thompson Sampling With Little to No Additional Computation

Thompson sampling has become a ubiquitous approach to online decision problems with bandit feedback. The key algorithmic task for Thompson sampling is drawing a sample from the posterior of the optimal action. We propose an alternative arm selection rule we dub TS-UCB, that requires negligible additional computational effort but provides significant performance improvements relative to Thompson sampling. At each step, TS-UCB computes a score for each arm using two ingredients: posterior sample(s) and upper confidence bounds. TS-UCB can be used in any setting where these two quantities are available, and it is flexible in the number of posterior samples it takes as input. TS-UCB achieves materially lower regret on a comprehensive suite of synthetic and real-world datasets, including a personalized article recommendation dataset from Yahoo! and a suite of benchmark datasets from a deep bandit suite proposed in Riquelme et al. (2018). Finally, from a theoretical perspective, we establish optimal regret guarantees for TS-UCB for both the K-armed and linear bandit models.

==> sections/regret_analysis_informs.tex <==

For our analysis, we introduce lower confidence bounds $(L_t)_{t \geq 1}$, which we define in a symmetric way to upper confidence bounds:
\begin{align} \label{def:lcb}
L_t(a) \triangleq \hmu_t(a) - (U_t(a) - \hmu_t(a)).
\end{align}

\subsection{Known Results}
We first state three known results used in the analysis. The first result says that the confidence bounds are valid with high probability.
\begin{lemma} \label{lem:hoeffding_general}
% For any $t$, $\Pr(\cup_{a \in \cA} \{\ft(a) \in [L_t(a), U_t(a)]\}) \leq 1/T$.
Using the functions $\{\hmu_t\}_{t \geq 1}$, $\{U_t\}_{t \geq 1}$ as defined in \eqref{eq:karmucb} in the $K$-armed setting and \eqref{eq:linearucb} in the linear bandit setting,
for any $t$, $\Pr(\ft(A) < U_t(A)) \leq T^{-3}$, where $A$ is any deterministic or random action.
The analogous bounds hold for the lower confidence bounds as defined in \eqref{def:lcb}, i.e. $\Pr(\ft(A) > L_t(A)) \leq T^{-3}$.
% The same analogous bounds hold for the lower confidence bounds $\{L_t\}_{t \geq 1}$
\end{lemma}
For completeness, the proof of Lemma~\ref{lem:hoeffding_general} can be found in Section~\ref{subsub:provelemmas}.
The following corollary is immediate using the law of total expectation and the fact that $\ft(A) > -1$.
\begin{corollary} \label{corr:lcb}
$\bE[- \ft(A)] \leq \bE[- L_t(A)] + T^{-3}$, where $A$ is any deterministic or random action.
% \begin{align}
% \bE[- \ft(A_t)] \leq \bE[- L_t(A_t)] + T^{-3}.
% \end{align}
\end{corollary}

The next two results upper bound $\sumt \bE[\rad_t(A_t)]$.
In particular, for the $K$-armed setting, the proof of Proposition 2 of \cite{russo2014learning} implies the following result.
\begin{theorem} \label{thm:sqrtbound}
For the $K$-armed bandit, using the UCBs as defined in \eqref{eq:karmucb},
\begin{align*}
\sumtK \bE[\rad_t(A_t)] \leq 2 \sqrt{3KT \log T },
\end{align*}
for any sequence of actions $A_t$.
\end{theorem}


Similarly, in the linear bandit setting, the proof of Theorem 3 of \cite{abbasi2011improved} (using the parameters $\delta=T^{-3}, \lambda=1$) implies the following result.
\begin{theorem} \label{thm:sqrtbound_linear}
For the linear bandit, using the UCBs as defined in \eqref{eq:linearucb},
\begin{align*}
% \sumt \bE[\rad_t(A_t)] \leq O(d \log T \sqrt{T}),
\sumt \bE[\rad_t(A_t)] \leq& 4\sqrt{Td \log(1+TL/d)}(S+ \subg \sqrt{6 \log(T) + d \log(1 + T/d)}) = O(d \log T \sqrt{T})
% =& O(d \log T \sqrt{T})
\end{align*}
for any sequence of actions $A_t$.
\end{theorem}

% Note that the upper bounds in Theorems~\ref{thm:sqrtbound} and \ref{thm:sqrtbound_linear} is of the same order as of Theorem~\ref{thm:mainK} and \ref{thm:mainlinear} repectively. Therefore, showing Theorems~\ref{thm:mainK} and \ref{thm:mainlinear} boil down to showing $\BReg(T, \pi^{\TSUCBE}) \leq C \sumt \bE[\rad_t(A_t)] + O(\sqrt{T})$ for a constant $C$.

% START PROOF
\subsection{Proof of Main Result}

There are two main steps of the proof which are stated in the following two propositions. These results apply to both the $K$-armed and linear bandit settings.

\begin{proposition} \label{thm:maingenerale}
Suppose $\rad_t(a) \in [\rmin, \rmax]$ for all $a \in \cA$ and $t \geq 1$.
Using the UCBs as defined in \eqref{eq:karmucb} for the $K$-armed bandit, and \eqref{eq:linearucb} for the linear bandit,
% \begin{align}
% \BReg(T, \pi^{\TSUCBE})   \leq  2 \sumt \bE[\rad_t(A_t)] + T^{-1} +  \frac{\rmax}{\rmin}.
% \end{align}
\begin{align} \label{eq:prop1}
 \BReg(T, \pi^{\TSUCB}) &\leq 2 \sumt \bE[\rad_t(\At)] + \frac{\rmax}{\rmin} \left(1+ \frac{2T}{\sqrt{m}} \right) + T^{-2}.
\end{align}
\end{proposition}

\begin{proposition} \label{thm:maingeneral}
Using the UCBs as defined in \eqref{eq:karmucb} for the $K$-armed bandit, and \eqref{eq:linearucb} for the linear bandit,
\begin{align*}
\BReg(T, \pi^{\TSUCB}) \leq  2 \sumt \bE[\rad_t(\At)] + (m+1)T^{-2}.
\end{align*}
\end{proposition}


The proof sketch from Section~\ref{sec:pfsketch} refers to the proof of Proposition~\ref{thm:maingenerale}. The approximation $\tf_t \approx \bE[\ft(\ssA) | H_t]$ used in the proof sketch only holds when $m$ is large; the fact that this doesn't hold contributes to the $\frac{1}{\sqrt{m}}$ term in \eqref{eq:prop1}, which goes to zero as $m \rightarrow \infty$.
Proposition~\ref{thm:maingeneral} has the opposite relationship with respect to $m$, so it applies when $m$ is small.
The final step of showing Theorems~\ref{thm:mainK} and \ref{thm:mainlinear} involves combining these two propositions to remove the dependence on $m$, showing $\frac{\rmax}{\rmin} = O(\sqrt{T})$, and plugging in the known bounds for $\sumt \bE[\rad_t(A_t)] $ from Theorems~\ref{thm:sqrtbound} and \ref{thm:sqrtbound_linear}.
Details of this final step are in Section~\ref{sec:combine}.

% We also often use the fact that $\ft(a) \leq 1$ in both settings, which implies $\tf \leq 1$ as well.

% MAIN PROOF
\subsubsection{Proof of Proposition~\ref{thm:maingenerale}.}
We first show the result claimed in \eqref{eq:tsucb_less_randomized}
whose proof is deferred to Section~\ref{subsub:provelemmas}.
\begin{lemma} \label{lem:random}
For any distribution $\tau$ over $\cA$,
 $\Psi_t(\At) \leq \bPsi_t(\tau)$ almost surely.
\end{lemma}
Next, we upper bound the ratio $\Psi_t(\At)$ by analyzing the Thompson Sampling policy.
\begin{lemma} \label{prop:boundratio}
$\Psi_t(\At) \leq 1 + \frac{1}{\rmin}(\Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t) +  \tf_t - \bE[f_{\theta}(\ssA)|H_t])$ almost surely.
Equivalently, using \eqref{eq:defratio1},
\begin{align} \label{eq:boundratio}
\tf_t - \hmu_{t}(\At)
\leq \rad_t(\At)(1 + \frac{1}{\rmin}(\Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t) +  \tf_t - \bE[f_{\theta}(\ssA)|H_t])).
\end{align}
\end{lemma}
\proof{Proof.}
Let $\pi^{\TSalg}$ be the Thompson sampling policy.
We show the inequality for $\bPsi_t(\pi_t^{\TSalg})$ instead, and then use $\Psi_t(\At) \leq \bPsi_t(\pi_t^{\TSalg})$ from Lemma~\ref{lem:random} to get the desired result.

% , and let $A_t$ be the action chosen by TS at time $t$.
By definition of TS,
$\pi_t^{\TSalg} = \pi_t^{\TSalg}(H_t)$ is the distribution over $\cA$ corresponding to the posterior distribution of $\ssA$ conditioned on $H_t$.
Then, if $A_t$ is the action chosen by TS at time $t$,
we have $\bE[U_t(A_t) |H_t] = \bE[U_t(\ssA)|H_t]$ and $\bE[\hmu_t(A_t) |H_t] = \bE[\hmu_t(\ssA)|H_t]$.
Using this, we can write $\bPsi_t(\pi_t^{\TSalg})$ as
\begin{align} \label{eq:psi_ts}
\bPsi_t(\pi_t^{\TSalg}) = \frac{\tf_t - \bE[\hmu_{t}(A_t)|H_t]}{\bE[U_t(A_t) - \hmu_{t}(A_t)|H_t]}
= \frac{\tf_t - \bE[\hmu_{t}(\ssA)|H_t]}{\bE[U_t(\ssA) - \hmu_{t}(\ssA)|H_t]}.
\end{align}

By conditioning on the event $\{f_{\theta}(\ssA) \leq U_t(\ssA)\}$, the following inequality follows from the fact that $f_{\theta}(\ssA) \leq 1$.
\begin{align} \label{eq:boundratiopf}
\bE[f_{\theta}(\ssA) | H_t] \leq \bE[U_t(\ssA)|H_t] + \Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t).
\end{align}
% Using this inequality and $\bE[U_t(A_t) |H_t] = \bE[U_t(\ssA)|H_t]$, we have
Consider the numerator of \eqref{eq:psi_ts}. We add and subtract $\bE[f_{\theta}(\ssA)|H_t]$ and use \eqref{eq:boundratiopf}:
\begin{align}
\tf_t - \bE[\hmu_{t}(\ssA)|H_t] &= \bE[f_{\theta}(\ssA)-\hmu_{t}(\ssA)|H_t]  + \tf_t - \bE[f_{\theta}(\ssA)|H_t] \nonumber \\
 &\leq \bE[U_t(\ssA) - \hmu_{t}(\ssA)|H_t] + \Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t) +  \tf_t - \bE[f_{\theta}(\ssA)|H_t]. \label{eq:boundratiopf2}
\end{align}
The first term of \eqref{eq:boundratiopf2} is equal to the denominator of $\bPsi_t(\pi^{\TSalg})$.
Therefore,
\begin{align*}
 \bPsi_t(\pi^{\TSalg})
 %  &= \frac{  \tf_t - \bE[\hmu_{t}(A_t)|H_t] }{\bE[U_t(A_t) - \hmu_{t}(A_t)|H_t]} \\
 % &= \frac{ \bE[f_{\theta}(\ssA)-\hmu_{t}(A_t)|H_t]  + \tf_t - \bE[f_{\theta}(\ssA)|H_t]}{\bE[U_t(A_t) - \hmu_{t}(A_t)|H_t]}  \\
 % &\leq \frac{\bE[U_t(\ssA) - \hmu_{t}(A_t)|H_t] + \Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t) +  \tf_t - \bE[f_{\theta}(\ssA)|H_t]}{\bE[U_t(\ssA) - \hmu_{t}(A_t)|H_t]} \\
             &\leq 1 + \frac{\Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t) +  \tf_t - \bE[f_{\theta}(\ssA)|H_t]}{\bE[U_t(\ssA) - \hmu_{t}(\ssA)|H_t]} \\
             &\leq 1 + \frac{1}{\rmin}(\Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t) +  \tf_t - \bE[f_{\theta}(\ssA)|H_t]).
\end{align*}
\endproof

% We now prove the main result, which involves applying Lemma~\ref{prop:boundratio} and some algebraic manipulations.

The next lemma simplifies the expectation of \eqref{eq:boundratio} using Cauchy-Schwarz.

\begin{lemma}\label{lem:mainlem}
For any $t$, $\bE[\tf_t - \hmu_{t}(\At)] \leq \bE[\rad_t(\At)]  + \frac{\rmax}{\rmin} \left(\frac{1}{T} + \frac{2}{\sqrt{m}} \right)$.
\end{lemma}

\proof{Proof.}

Taking the expectation of \eqref{eq:boundratio} gives us
\begin{align}
\bE[\tf_t - \hmu_{t}(\At)]
\leq& \bE[\rad_t(\At)(1 + \frac{1}{\rmin}(\Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t) +  \tf_t - \bE[f_{\theta}(\ssA)|H_t]))] \nonumber \\
=& \bE[\rad_t(\At)] \nonumber \\
 &+\frac{1}{\rmin}\bE[\rad_t(\At)\Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t)] \label{eq:firstcs} \\
 & +  \frac{1}{\rmin}\bE[\rad_t(\At) (\tf_t - \bE[f_{\theta}(\ssA)|H_t])]. \label{eq:secondcs}
\end{align}

We will now upper bound \eqref{eq:firstcs} and \eqref{eq:secondcs} with $\frac{\rmax}{\rmin} \cdot \frac{1}{T}$ and $\frac{\rmax}{\rmin} \cdot \frac{2}{\sqrt{m}}$ respectively, in which case the result will follow.
First, consider \eqref{eq:firstcs}. Using Cauchy-Schwarz yields
\begin{align}
 &\frac{1}{\rmin} \bE[\rad_t(\At)\Pr(f_{\theta}(\ssA) > U_t(\ssA) | H_t)]  \\
 \leq& \frac{1}{\rmin}  \sqrt{\bE[\rad_t(\At)^2] \bE[\Pr(\ft(\ssA) > U_t(\ssA) | H_t)^2]} \nonumber \\
 \leq& \frac{1}{\rmin T}\sqrt{\bE[\rad_t(\At)^2]} \nonumber \\
 \leq& \frac{1}{T} \cdot \frac{\rmax}{\rmin}, \label{eq:cs1}
\end{align}
where the second step uses the following.
\begin{align}
\bE[\Pr(\ft(\ssA) > U_t(\ssA) | H_t)^2] &= \bE[\bE[\bI(\ft(\ssA) > U_t(\ssA)) | H_t]^2] \nonumber \\
&\leq \bE[\bE[\bI(\ft(\ssA) > U_t(\ssA))^2 | H_t]] \nonumber \\
 &=\bE[\bE[\bI(\ft(\ssA) > U_t(\ssA)) | H_t]] \nonumber \\
&\leq  \Pr(\ft(\ssA) > U_t(\ssA)) \nonumber \\
&\leq \frac{1}{T^2}, \label{eq:uncondprob}
\end{align}
where the first inequality uses Jensen's inequality, and the last inequality uses Lemma~\ref{lem:hoeffding_general}.

Similarly, we apply Cauchy-Schwarz to \eqref{eq:secondcs}.
\begin{align}
 \frac{1}{\rmin}\bE[\rad_t(\At) (\tf_t - \bE[f_{\theta}(\ssA)|H_t])] &\leq \frac{1}{\rmin}\sqrt{\bE[\rad_t(\At)^2] \bE[(\tf_t - \bE[f_{\theta}(\ssA)|H_t])^2]}. \label{eq:cs2mid}
\end{align}

Recall that $\tf_t = \frac{1}{m} \sum_{i = 1}^m \tf_i$, and $\tf_i$ has the same distribution as $f_{\theta}(\ssA)$ conditioned on $H_t$.
Therefore, $\bE[\tf_t|H_t] = \bE[f_{\theta}(\ssA)|H_t]$. Then, we have
% \begin{align}
%  \bE[\rad_t(A_t) (\tf_t - \bE[f_{\theta}(\ssA)|H_t])] &\leq \sqrt{\bE[\rad_t(A_t)]^2 \bE[\bE[(\tf_t - \bE[f_{\theta}(\ssA)|H_t])^2|H_t]]} \\
%       &\leq \sqrt{\bE[\rad_t(A_t)]^2 \bE[\var(\tf_t | H_t)]}.
%       &\leq \sqrt{\bE[\rad_t(A_t)]^2 \bE[\var(\tf_t | H_t)]}.
% \end{align}
\begin{align}
\bE[(\tf_t - \bE[f_{\theta}(\ssA)|H_t])^2] &= \bE[\bE[(\tf_t - \bE[f_{\theta}(\ssA)|H_t])^2|H_t]] \nonumber \\
&= \bE[\var(\tf_t | H_t)] \nonumber \\\
&= \bE[\frac{1}{m}\var(\tf_i | H_t)] \nonumber  \\\
&\leq \frac{4}{m}. \nonumber % \label{eq:var}
\end{align}
The last inequality follows since $\tf_i \in [-1, 1]$.
Combining this with \eqref{eq:cs2mid}, we get
\begin{align}
 \frac{1}{\rmin}\bE[\rad_t(\At) (\tf_t - \bE[f_{\theta}(\ssA)|H_t])] &\leq \frac{2}{\rmin\sqrt{m}} \sqrt{\bE[\rad_t(\At)^2]} \nonumber \\
                            &\leq \frac{2}{\sqrt{m}} \cdot \frac{\rmax}{\rmin} \label{eq:cs2}
\end{align}

Substituting \eqref{eq:cs1} and \eqref{eq:cs2} into \eqref{eq:secondcs} yields the desired result.
% \begin{align}
% \bE[\tf_t - \hmu_{t}(A_t)] = \bE[\rad_t(A_t)]  + \frac{\rmax}{\rmin} \left(\frac{1}{T} + \frac{2}{\sqrt{m}} \right)
% \end{align}
\Halmos
\endproof

% END PROOF
\proof{Proof of Proposition~\ref{thm:maingenerale}.}
Conditioned on $H_t$, the expectation of $\ft(\ssA)$ and $\tf_t$ is the same, implying $\bE[\ft(\ssA)] = \bE[\tf_t]$ for any $t$. Therefore, the Bayes regret can be written as $\sumt \bE[\tf_t- \ft(\At)]$.
By adding and subtract $\hmu_t(\At)$, we derive
\begin{align}
 \BReg(T, \pi^{\TSUCBE}) =& \sumt \bE[\tf_t - \hmu_{t}(\At)] + \sumt \bE[\hmu_{t}(\At)- \ft(\At)]. \label{eq:decomp1}
\end{align}

% Using $\bE[\ft(\ssA)] = \bE[\tf_t]$ for all $t$,
% we add and subtract $\mu_t(A_t)$ to the Bayes regret to derive
% \begin{align}
%  \BReg(T, \pi^{\TSUCBE})   =& \sumt \bE[\ft(\ssA) - \ft(A_t)] \nonumber \\
%                  =& \sumt \bE[\tf_t- \ft(A_t)] \nonumber \\
%               =& \sumt \bE[\tf_t - \hmu_{t}(A_t)] + \sumt \bE[\hmu_{t}(A_t)- \ft(A_t)]. \label{eq:decomp1}
% \end{align}

% We will show that each of the two sums in \eqref{eq:decomp1} are of order $O(\sqrt{KT\log T})$.
The first sum in \eqref{eq:decomp1} can be bounded by $\sumt \bE[\rad_t(\At)]  + \frac{\rmax}{\rmin} \left(1 + \frac{2T}{\sqrt{m}} \right)$ using Lemma~\ref{lem:mainlem}.
Using Corollary~\ref{corr:lcb}, the second sum in \eqref{eq:decomp1} can be bounded by
$\sumt (\bE[\hmu_{t}(\At)- L_t(\At)] +  T^{-3}) \leq \sumt \bE[\rad_t(\At)] + T^{-2}$.
% \begin{align*}
% \sumt \bE[\hmu_t(\At)- \ft(\At)] \leq& \sumt (\bE[\hmu_{t}(\At)- L_t(\At)] +  T^{-3}) \nonumber \\
%                   \leq& \sumt \bE[\rad_t(\At)] + T^{-2}.  \label{eq:firstterm}
% \end{align*}
Substituting these two bounds results in
\begin{align*}
 \BReg(T, \pi^{\TSUCBE}) &\leq 2 \sumt \bE[\rad_t(\At)] + \frac{\rmax}{\rmin} \left(1+ \frac{2T}{\sqrt{m}} \right) + T^{-2}
\end{align*}
as desired.
\Halmos
\endproof

\subsubsection{Proof of Proposition~\ref{thm:maingeneral}.}

The main idea of this proof is captured in the following lemma, which says that we can essentially replace the term $\bE[f_\theta(\ssA)]$ with $\bE[U_{t}(\At)]$.
\begin{lemma} \label{lem:ucbratioone2}
% $\bE[f_\theta(\ssA)] \leq \bE[U_t(\At)] + \Pr(f_\theta(\ssA) > \max_{a \in \cA} U_t(a))$.
For every $t$, $\bE[f_\theta(\ssA)] \leq \bE[U_{t}(\At)] + mT^{-3}$.
\end{lemma}
\proof{Proof.}
Fix $t$, $H_t$, and $\tf_t$.
For an action $a \in \cA$,
if $U_{t}(a) \geq \tf_t$, then $\Psi_{t}(a) \leq 1$ since the denominator of the ratio is always positive.
Otherwise, if $U_t(a) < \tf_t$, then $\Psi_t(a) > 1$.
This implies that an action whose UCB is higher than $\tf_t$ will always be chosen over an action whose UCB is smaller than $\tf_t$.
Therefore, in the case that $\tf_t \leq \max_{a \in \cA} U_t(a)$, it will be that $U_t(\At) \geq \tf_t$.
% Otherwise, if $\tilde{f}_t > \max_{a \in \cA} U_t(a)$, then
Since $\tf_t \leq 1$, we have
\begin{align*}
\bE[\tf_t |  H_t ] \leq \;&U_t(\At) \Pr(\tf_t\leq \max_{a \in \cA} U_t(a) | H_t ) + \Pr(\tf_t> \max_{a \in \cA} U_t(a) | H_t ) \\
              \leq \; & U_t(\At) + \Pr(\tf_t > \max_{a \in \cA} U_t(a) | H_t ) .
\end{align*}
Since $\tf_t = \frac{1}{m} \sum_{i = 1}^m \tf_i$, if $\tf_t$ is larger than $\max_{a \in \cA} U_t(a)$, it must be that at least one of the elements $\tf_i$ is larger than $\max_{a \in \cA} U_t(a)$.
Then, the union bound gives us $\Pr(\tf_t > \max_{a \in \cA} U_t(a) | H_t ) \leq \sum_{i = 1}^m \Pr(\tf_i > \max_{a \in \cA} U_t(a) | H_t )$.
By definition of $\tf_i$, the distribution of $\tf_i$ and $\ft(\ssA)$ are the same conditioned on $H_t$.% Moreover, $\bE[\tf | H_t] = \bE[\ft(\ssA)|H_t]$.
Therefore,
\begin{align*}
\bE[\tf_t |  H_t ] \leq  U_t(\At) + m \Pr(\ft(\ssA) > \max_{a \in \cA} U_t(a) | H_t ).
\end{align*}

Using the fact that $\bE[\tf_t | H_t] = \bE[\ft(\ssA)|H_t]$ and taking expectations on both sides, we have
\begin{align*}
\bE[\ft(\ssA)] &\leq \bE[U_t(\At)] + m \Pr(\ft(\ssA) > \max_{a \in \cA} U_t(a)) \\
         &\leq \bE[U_t(\At)] + m \Pr(\ft(\ssA) >  U_t(\ssA)) \\
         &\leq \bE[U_t(\At)] + mT^{-3}.
\end{align*}
The last inequality uses Lemma~\ref{lem:hoeffding_general}.
\Halmos
\endproof

% \begin{proposition} \label{thm:1sampleradius}
% $\BReg(T, \pi^{\TSUCB}) \leq \sumt 2\bE[\rad_t(\At)] + 2mT^{-1}$.
% \end{proposition}

\proof{Proof of Proposition~\ref{thm:maingeneral}.}
% First, we use Lemma~\ref{lem:ucbratioone2} to write
\begin{align*}
 \BReg(T, \pi^{\TSUCB}) &= \sumt \bE[\ft(\ssA) - \ft(\At)] \\
              &\leq \sumt (\bE[U_t(\At) - \ft(\At)]  + mT^{-3}) \\
              &\leq \sumt (\bE[U_t(\At) - L_t(\At)] + T^{-3})  + mT^{-2}\\
              &= 2 \sumt \bE[\rad_t(\At)]  + (m+1)T^{-2},
\end{align*}
where the first inequality uses Lemma~\ref{lem:ucbratioone2} and the second inequality uses Corollary~\ref{corr:lcb}.
% Then, replacing the term $\bE[- \ft(A_t)]$ with $\bE[- L_t(A_t)] + T^{-3}$ using Corollary~\ref{corr:lcb} completes the proof.
% \begin{align*}
%  \BReg(T, \pi^{\TSUCB}) \leq& \sumt (\bE[U_t(A_t) - L_t(A_t)] + T^{-3})  + mT^{-2}\\
%               \leq& 2 \sumt \bE[\rad_t(A_t)]  + (m+1)T^{-2},
% \end{align*}
% as required.
\Halmos
\endproof

% COMBINE
\subsubsection{Final step of proof.} \label{sec:combine}

\proof{Proof of Theorem~\ref{thm:mainK}.}

The UCBs in \eqref{eq:karmucb} imply that $\rad_t(a) \in [\sqrt{\frac{3 \log T}{T}}, \sqrt{3 \log T}]$ for all $a$ and $t$, therefore $\frac{\rmax}{\rmin} \leq \sqrt{T}$.
Then, Propositions~\ref{thm:maingenerale} and \ref{thm:maingeneral} result in the following two inequalities respectively:
\begin{align*}
 \BReg(T, \pi^{\TSUCB}) &\leq 2 \sumt \bE[\rad_t(\At)] + \sqrt{T} + 2\sqrt{\frac{T^{3}}{m}} + T^{-2}, \\
 \BReg(T, \pi^{\TSUCB}) &\leq  2 \sumt \bE[\rad_t(\At)] + \frac{m}{T^2} + T^{-2}.
\end{align*}
Combining these two bounds results in
\begin{align*}
 \BReg(T, \pi^{\TSUCB}) \leq  2 \sumt \bE[\rad_t(\At)] + \sqrt{T} +  T^{-2} +\min\left\{2\sqrt{\frac{T^{3}}{m}}, \frac{m}{T^2}\right\}.
\end{align*}
For any value of $m > 0$, $\min\left\{2\sqrt{\frac{T^{3}}{m}}, \frac{m}{T^2}\right\} \leq 2\sqrt{T}$. Plugging in the known bound for $\sumt \bE[\rad_t(\At)]$ from Theorem~\ref{thm:sqrtbound} finishes the proof of Theorem~\ref{thm:mainK}.\footnote{The statement of Theorem~\ref{thm:mainK} has an additional $+ K$ term since the first $K$ time steps are used to pull each arm once, which we did not include in the proof to simplify exposition.}.
% Combining Proposition~\ref{thm:sqrtbound} with \ref{thm:maingenerale} give us Theorem~\ref{thm:mainK}.
\Halmos
\endproof


\proof{Proof of Theorem~\ref{thm:mainlinear}.}
% For the linear bandit, \eqref{eq:mainlinear} follows from Proposition~\ref{thm:maingenerale}.
The following lemma, whose proof is deferred to Section~\ref{subsub:provelemmas}, allows us to bound $\frac{\rmax}{\rmin}$ by $4\sqrt{2T}$.
% Combining Theorem~\ref{thm:sqrtbound_linear} with Proposition~\ref{thm:maingeneral} implies \eqref{eq:mainlinear} of Theorem~\ref{thm:mainlinear}.
% % For the linear bandit, we can show that $\frac{\rmax}{\rmin} \leq 4\sqrt{2T}$ using the following lemma.
% The following lemma, whose proof is deferred to Section~\ref{subsub:provelemmas}, allows us to bound $\frac{\rmax}{\rmin}$ by $4\sqrt{2T}$ in the linear bandit setting.
\begin{lemma} \label{lem:linradiusbounds}
For the linear bandit, using the UCBs as defined in \eqref{eq:linearucb}, if $||X(a)||_2 =1$ for every $a$, then $\rad_t(a) \in [\subg\sqrt{\frac{d \log T}{T}}, 4\subg\sqrt{2 d \log T}]$ for every $t$ and $a$.
\end{lemma}

Then, using the same steps from the proof of Theorem~\ref{thm:mainK}, we derive
\begin{align}
 \BReg(T, \pi^{\TSUCB}) \leq 2 \sumt \bE[\rad_t(\At)] + 4\sqrt{2T} +  T^{-2} +\min\left\{8 \sqrt{\frac{2T^{3}}{m}}, \frac{m}{T^2}\right\}.
\end{align}

For any $m$, $\min\left\{8 \sqrt{\frac{2T^{3}}{m}}, \frac{m}{T^2}\right\} \leq 8 \sqrt{2T}$. Plugging in the known bound for $\sumt \bE[\rad_t(\At)]$ from Theorem~\ref{thm:sqrtbound_linear} gives us \eqref{eq:mainlineare}, finishing the proof of Theorem~\ref{thm:mainlinear}.
\Halmos
\endproof

% LEMMAS
\subsection{Proofs of Lemmas} \label{subsub:provelemmas}

\proof{Proof of Lemma~\ref{lem:random}.}
Fix $H_t$ and $\tf_t$. For every action $a$, let $\Delta_a = \tf_t - \hmu_t(a)$, and hence $\Psie_t(a) = \frac{\Delta_a}{\rad_t(a)}$.
% Let $p$ be a randomized policy such that assigns probability $p_a$ to action $a$.
Let $\nu$ be a distribution over $\cA$.
Then,
\begin{align} \label{eq:lemrand}
\bPsi_t(\nu)  = \frac{\bE_{a \sim \nu}[\Delta_a]}{ \bE_{a \sim \nu}[\rad_t(a)]}.
\end{align}
$\rad_t(a)> 0$ for all $a$, but $\Delta_a$ can be negative.
We claim that the above ratio is minimized when $\tau$ puts all of its mass on one action ---
in particular, the action $\ssa \in \argmin_a \frac{\Delta_a}{\rad_t(a)}$.

For $a \neq \ssa$, let $c_a = \frac{\rad_t(a)}{\rad_t(\ssa)} > 0$.
Then, since $\Psie_t(a) \geq \Psie_t(\ssa)$, we can write
$\Delta_a = c_a\Delta_{\ssa} + \delta_a$ for $\delta_a \geq 0$ for all $a$.
Let $p_{\ssa} = \Pr(a = \ssa)$.
Let $E = \{a \neq \ssa\}$
Substituting into \eqref{eq:lemrand}, we get
\begin{align*}
\bPsi_t(\nu)
&= \frac{\bE[c_a\Delta_{\ssa} + \delta_a]}
        {\bE[c_a \rad_t(\ssa)]} \\
&= \frac{p_{\ssa}\Delta_{\ssa} + \bE[c_a\Delta_{\ssa} + \delta_a|E]\Pr(E)}
        {p_{\ssa} \rad_t(\ssa) +  \bE[c_a \rad_t(\ssa)|E]\Pr(E)} \\
&= \frac{\Delta_{\ssa}\left(p_{\ssa} + \bE[c_a|E]\Pr(E)\right) + \bE[\delta_a|E]\Pr(E)}
        { \rad_t(\ssa)\left( p_{\ssa}+  \bE[c_a|E]\Pr(E)\right)} \\
&= \frac{\Delta_{\ssa}} { \rad_t(\ssa)} +
   \frac{\bE[\delta_a|E]\Pr(E)}{\rad_t(\ssa)\left( p_{\ssa}+  \bE[c_a|E]\Pr(E)\right)} \\
&\geq \frac{\Delta_{\ssa}} { \rad_t(\ssa)} \\
&= \Psi_t(\ssa)
\Halmos
\end{align*}
\endproof
\proof{Proof of Lemma~\ref{lem:hoeffding_general}.}
In the linear bandit, this lemma follows directly from Theorem 2 of \cite{abbasi2011improved} (using the parameters $\delta=T^{-3}, \lambda=1$).
In the $K$-armed setting, if $\hmu(n, a)$ is the empirical mean of the first $n$ plays of action $a$, Hoeffding's inequality implies $\Pr(\ft(a) - \hmu(n, a) \geq  \sqrt{\frac{3 \log T}{n}} ) \leq T^{-6}$ for any $n$.
Then, since the number of plays of a particular action is no larger than $T$, we have
\begin{align*}
\Pr(\ft(a) - \hmu_t(a) \geq \sqrt{\frac{3 \log T}{N_t(a)}}) &\leq \Pr(\cup_{n=1}^T \{\ft(a) - \hmu(n, a) \geq \sqrt{\frac{3 \log T}{n}}\}) \leq  T^{-5}.
\end{align*}
Since $|\cA| = K \leq T$ and $\ssA, A_t \in \cA$, the result follows after taking another union bound over actions (which proves a stronger bound of $T^{-4}$).
\Halmos
\endproof

\proof{Proof of Lemma~\ref{lem:linradiusbounds}.}
We have
\begin{align*}
\rad_t(a) = \sqrt{\beta_t} || X(a)||_{V_t^{-1}}= \sqrt{\beta_t} ||V_t^{-1/2} X(a)||_2.
\end{align*}
Then, since $||X(a)||_2 = 1$ for all $a$,
\[
\sqrt{\beta_t}\sigma_{\min}(V_t^{-1/2}) \leq \rad_t(a) \leq \sqrt{\beta_t}\sigma_{\max}(V_t^{-1/2}).
\]


First, we lower bound $\sigma_{\min}(V_t^{-1/2})$.
To do this, we can instead upper bound $||V_t||_2$, since $\sigma_{\min}(V_t^{-1/2}) = \sqrt{\sigma_{\min}(V_t^{-1})} = \frac{1}{\sqrt{\sigma_{\max}(V_t)}} = \frac{1}{\sqrt{||V_t||_2}}$.
The triangle inequality gives $||V_t||_2 \leq || I ||_2 + \sum_{s = 1}^t ||X_s X_s^\top||_2$.
Since $X_s X_s^\top$ is a rank-1 matrix, the only non-zero eigenvalue is $||X_s||_2^2 = 1$ with eigenvector $X_s$, since $(X_s X_s^\top) X_s = X_s (X_s^\top X_s)$. Therefore, $||V_t||_2 \leq || I ||_2 + \sum_{s = 1}^t ||X_s||_2^2 \leq 1 + T$, which implies $\sigma_{\min}(V_t^{-1/2})  \geq \frac{1}{\sqrt{T+1}} \geq \frac{1}{\sqrt{2T}}$.
Recall $\sqrt{\beta_t} = \subg \sqrt{d \log(T^2(1+t))} + S \geq \subg \sqrt{d \log T}$, implying $\rad_t(a) \geq \subg \sqrt{\frac{d \log T}{2T}}$.
% \[
% \rad_t(a) \geq \sqrt{\beta_t}\sigma_{\min}(V_t^{-1/2}) \geq R \sqrt{ \frac{d \log T}{T}}.
% \]

Next, we upper bound $\sigma_{\max}(V_t^{-1/2}) = \frac{1}{\sqrt{\sigma_{\min}(V_t)}}$ by lower bounding $\sigma_{\min}(V_t)$.
$\sigma_{\min}(V_t) \geq \sigma_{\min}(I) = 1$. Therefore, $\sigma_{\max}(V_t^{-1/2}) \leq 1$.
We can upper bound $\sqrt{\beta_t}$ by $\subg\sqrt{d \log(T^4)} + S \leq 2 \subg\sqrt{4d \log(T)}$, since we assumed $\subg \geq 1$ and $S \leq \sqrt{d}$.
Therefore, we have
\[
\rad_t(a) \leq \sqrt{\beta_t} \leq 4 \subg\sqrt{d \log(T)}.  \; \Halmos
\]
\endproof

